Structure Guided Prompt: Instructing Large Language Model in Multi-Step Reasoning by Exploring Graph Structure of the Text

Although Large Language Models (LLMs) excel at addressing straightforward reasoning tasks, they frequently struggle with difficulties when confronted by more complex multi-step reasoning due to a range of factors. Firstly, natural language often encompasses complex relationships among entities, making it challenging to maintain a clear reasoning chain over longer spans. Secondly, the abundance of linguistic diversity means that the same entities and relationships can be expressed using different terminologies and structures, complicating the task of identifying and establishing connections between multiple pieces of information. Graphs provide an effective solution to represent data rich in relational information and capture long-term dependencies among entities. To harness the potential of graphs, our paper introduces Structure Guided Prompt, an innovative three-stage task-agnostic prompting framework designed to improve the multi-step reasoning capabilities of LLMs in a zero-shot setting. This framework explicitly converts unstructured text into a graph via LLMs and instructs them to navigate this graph using task-specific strategies to formulate responses. By effectively organizing information and guiding navigation, it enables LLMs to provide more accurate and context-aware responses. Our experiments show that this framework significantly enhances the reasoning capabilities of LLMs, enabling them to excel in a broader spectrum of natural language scenarios.

==> content/limit.tex <==
\section{Limitations}
Our research does not introduce new ethical risks beyond those already present in the field of prompting-based reasoning. However, given that our work falls under the umbrella of LLMs, there is still a possibility that these models may produce unexpected reasoning outputs. We look forward to future developments in this area that may mitigate such concerns.

==> content/problem_definition.tex <==
\section{Graph Representation of Unstructured Text and Reasoning Task}
Humans often represent unstructured text as a graph to provide a more comprehensive and coherent overview of the relationships that exist among various entities. These becomes extremely useful especially when dealing with complex information. Within this graphical representation, each node corresponds to an entity, and the interconnecting edges depict the relationships linking these entities.

\subsection{Graph Construction over Unstructured Text}
Let's illustrate the process of constructing a graph from unstructured text using an example. Consider the following paragraph: ``Christian got his son, \textbf{{\color{red}Seth}}, a car for his birthday. Christian and his brother Jonathan went to a basketball game. Jonathan's sister Ruth decided to tag along with them. Ruth invited her daughter Stephanie to lunch. Stephanie's brother \textbf{{\color{red}Jeremy}} couldn't leave work to join them.'' In this context, our objective is to determine the family relationship between \textit{Seth} and \textit{Jeremy}. Since this question pertains to the kinship connections among individuals, we simplify the process of answering it by creating a kinship graph based on the information provided in the text. This graph captures all the relevant facts related to family relations, as illustrated in Fig.~\ref{fig:graph representation}.

\begin{figure}[h]
    \centering
    \includegraphics[width= \linewidth]{figure/Graph Representation.pdf}
    %\vspace{-2em}
    \caption{The graph representation of a story from CLUTRR dataset. our objective is to determine the family relationship between two nodes, \textit{Seth} and \textit{Jeremy}, which are highlighted in red. } 
    \label{fig:graph representation}
\end{figure}

From the graph in the Fig.~\ref{fig:graph representation}, we can observe that even though the text is concise and the question appears relatively straightforward, the graphical representation reveals a long path connecting \textit{Seth} and \textit{Jeremy}. To arrive at an accurate answer, we have to traverse the graph 
% $\text{Seth}\xleftarrow{\text{hasSon}}\text{Christian}\xrightarrow{\text{hasBrother}}\text{Jonathan}\xrightarrow{\text{hasSister}}\text{Ruth} \xrightarrow{\text{hasDaughter}}\text{Stephanie}\xrightarrow{\text{hasBrother}}\text{Jeremy}$ 
and perform inference step by step: Step 1:
Given $\text{Seth}\xleftarrow{\text{hasSon}}\text{Christian}\xrightarrow{\text{hasBrother}}\text{Jonathan}$, we have $\text{Seth}\xrightarrow{\text{hasUncle}}\text{Jonathan}$; Step 2:
Given $\text{Seth}\xrightarrow{\text{hasUncle}}\text{Jonathan} \xrightarrow{\text{hasSister}}\text{Ruth}$, we have $\text{Seth}\xrightarrow{\text{hasAunt}}\text{Ruth}$; Step 3:
Given $\text{Seth}\xrightarrow{\text{hasAunt}}\text{Ruth} \xrightarrow{\text{hasDaughter}}\text{Stephanie}$, we have $\text{Seth}\xrightarrow{\text{hasCousin}}\text{Stephanie}$; Step 4:
Given $\text{Seth}\xrightarrow{\text{hasCousin}}\text{Stephanie} \xrightarrow{\text{hasBrother}}\text{Jeremy}$, we have $\text{Seth}\xrightarrow{\text{hasCousin}}\text{Jeremy}$. 



==> content/task_old.tex <==
\section{Exploring Representative KG Reasoning Tasks}
% \KC{
% According to Yizhou, she doesn't like the current organization that divides downstream tasks into three categories and introduces each method separately. She prefers to introduce the framework's workflow instead. In essence, the workflow can be summarized as a three-step framework:
% 1 Building a Knowledge Graph (KG).
% 2 Define the task.
% 3 Defining atomic operations based on the specific downstream task and progressing step by step, guided by these atomic operations, until reaching the final answer.
% Furthermore, in her view, the current classification of downstream tasks is inadequate. She believes that Query Answering can be seen as a specialized case of entity prediction, making it challenging to clearly define these three downstream tasks within the scope of this paper.
% }
% As we discussed in the previous section, since we organize unstructured text into a Concept Map and aim to leverage this Concept Map for answering questions, it's crucial to recognize that various questions may necessitate distinct graph structures and thus require different planning. 
Our framework is inherently task-agnostic, designed to accommodate a wide range of tasks with versatility. To cater to this diversity, we establish task-specific planning in 2nd stage prompt, tailored to each unique task. This section outlines various planning approaches for different tasks, demonstrating the framework's adaptability.
% Considering that we organize unstructured text into a Knowledge Graph (KG) and aim to leverage this KG for answering questions, it's crucial to recognize that various questions may necessitate distinct graph structures and thus require different planning. 
% These structures can predominantly fall into two primary categories: (1) entity prediction and (2) relational prediction. To address this diversity, we introduce how \textbf{\model{}} effectively accommodate each of these tasks with flexibility.
We have provided all these prompts in Appendix A.2.
% \subsection{\model{}}
% We propose \model{}, a \textbf{zero-shot} template-based prompting to instructing LLMs in multi-hop reasoning by exploring the graph structure of text. It is inherently task-agnostic and elicits multi-hop reasoning across a wide range of tasks with a single template. The core idea of our method is simple, as described in introduction: add
% explicitly extracting structural information,
% represented as a Knowledge Graph (KG), from unstructured text

\subsection{Relation Prediction}
Relation prediction is a task focused on predicting the missing relations between two given entities, represented as $(h, ?, t)$. This task typically involves inferring the missing relations by tracing the path that links the target entities (i.e., $h$ and $t$) within the graph. We have discussed the planning strategies applicable to relation prediction task in Sec.~\ref{sec:Frameworks}.
% Relational reasoning can involve deductive and inductive reasoning to derive new knowledge from existing facts in the KG. Deductive reasoning is a process of deriving specific conclusions from general principles or known facts. For example, if the KG contains information that A is the parent of B and B is the parent of C, one can infer that A is the grandparent of C. Inductive reasoning, on the other hand, is the process of making generalized conclusions based on specific observations or patterns in data. For example, 
% \begin{tcbraster}[raster equal height,raster valign=top,raster columns=2, raster rows=1, colback=white,colframe=white]
% \begin{tcolorbox}[title = Deductive Reasoning,colback=blue!5!white,colframe=blue!75!black,fonttitle=\bfseries,height=4cm, width = 8cm]
% Premise 1: A is the parent of B.
% Premise 2: B is the parent of C.
% Conclusion: Therefore, A is the grandparent of C.
% \end{tcolorbox}
% \begin{tcolorbox}[title = Inductive Reasoning,colback=blue!5!white,colframe=blue!75!black,fonttitle=\bfseries,height=4cm, width = 4cm]
% Observation 1: Crow A is black.
% Observation 2: Crow B is black.
% Observation 3: Crow C is black.
% Conclusion: Therefore, all crows are black.
% \end{tcolorbox}
% \end{tcbraster}
% Consider the following question: 

% ``QUESTION: Stanley took his granddaughter Darnell to the movies. Marian's sister Valerie was trying on new make-up that Marian's daughter Darnell bought for her as a gift. What is the family relationship between Valerie and Stanley?'' CORRECT ANSWER: daughter. 

% In this context, our objective is to determine the family relationship between \textit{Valerie} and \textit{Stanley}, which isn't directly mentioned in the story. Given the absence of direct information regarding the family link between Valerie and Stanley, ChatGPT-3.5, without prompt engineering, cannot definitively determine their precise familial connection. However, by transforming the unstructured text into a Knowledge Graph (KG) and instructing ChatGPT-3.5 to traverse from the subject entity to the object entity step by step to address the question, we can observe ChatGPT-3.5 navigating a path: $\textbf{{\color{red}Stanley}}\xrightarrow{\text{hasGranddaughter }}\textbf{{\color{green}Darnell}}\xrightarrow{\text{hasMother}}\textbf{{\color{blue}Marian}}\xrightarrow{\text{hasSister}}\textbf{{\color{brown}Valerie}}$. Following this path allows us to conclude that the family relationship between Valerie and Stanley is that Valerie is Stanley's daughter.

% \begin{tcbraster}[raster equal height,raster valign=top,raster columns=1, raster rows=1, colback=white,colframe=white]
% \begin{tcolorbox}[title = 0-CoT ,colback=green!5!white,colframe=green!75!black,fonttitle=\bfseries,height=4cm]
% In the given story, \hl{there is no direct information provided about the family relationship between Valerie and Stanley}. Therefore, based solely on the provided story, we cannot determine the exact family relationship between Valerie and Stanley.

% \end{tcolorbox}
% \begin{tcolorbox}[title = \model{},colback=green!5!white,colframe=green!75!black,fonttitle=\bfseries,height=12cm]
% Certainly, let's break down the story and use inductive reasoning to answer the question about the family relationship between \textit{Valerie} and \textit{Stanley}.

% \textbf{{\color{red}Stanley}}: The story starts with Stanley. He took his granddaughter \textbf{{\color{green}Darnell}} to the movies.

% \textbf{{\color{green}Darnell}}: Darnell is Stanley's granddaughter. \hl{This establishes Stanley's role as a grandfather.}

% \textbf{{\color{blue}Marian}}: Although not directly mentioned in relation to Stanley, we know that \textbf{{\color{blue}Marian}} is somehow connected to \textbf{{\color{green}Darnell}} because she is Darnell's mother. This means that \hl{Marian is Stanley's daughter.}

% \textbf{{\color{brown}Valerie}}: The story mentions \textbf{{\color{brown}Valerie}} as \textbf{{\color{blue}Marian}}'s sister. This means that \hl{Valerie is also Stanley's daughter}, making her his daughter as well.

% So, inductive reasoning leads us to conclude that the family relationship between Valerie and Stanley is that \hl{Valerie is Stanley's daughter}.
% \end{tcolorbox}

% \end{tcbraster}




% The most representative dataset for relational reasoning is CLUTRR~\cite{sinha2019clutrr} (Compositional Language Understanding with Text-based Relational Reasoning). It is a benchmark designed to infer the relationship between two family members, which isn't directly mentioned in the story. Successful performance on this task requires both extracting relationships between entities, as well as inferring the logical rules governing these relationships.



\subsection{Entity Prediction}
\subsubsection{Simple Entity Prediction}
Entity prediction is a fundamental task in Knowledge Graphs (KGs) that aims to infer the missing entity in a given query, such as $(e_i, r_k, ?)$ or $(?, r_k, e_j)$. For example, the question ``Who currently holds the position of President in the USA?'' can be structured as a link prediction task within a KG, seeking to resolve the query $(?, \text{isPresidentOf}, \text{USA})$. This query could be straightforward, in this paper, we focus on more complex query which require multi-step for inference. Examples are given in the following paragraph. As knowledge within KGs can either remain static or evolve dynamically, each scenario presents unique implications for inference. Consequently, we distinguish between \textit{Static KGs} and \textit{Dynamic KGs}, addressing entity prediction within each scenario separately.

\textbf{Static KG}: A static KG typically contains facts and relationships that do not change over time. For example, a static KG can be exemplified through statements concerning scientific common sense, which is presented as follows:
% For example, ``Gravity causes orbits. Planets in the solar system orbit the sun.'' can be arranged as a static KG. 

\textit{QUESTION: ``Ocean is the largest body body of water on earth. Body of water is a source of wild fish for human populations. As the size of a body of water increases, the amount of wild fish will increase. Which of the following is the greatest source of wild fish for human populations?''
CORRECT ANSWER: Ocean} 

When posing this question to ChatGPT-3.5 without prompt engineering, the response provided is "the Pacific Ocean." We can observe that ChatGPT-3.5 provided the correct answer by relying more on general knowledge of the real world rather than relying on logical inference derived from the provided facts. However, upon structuring the paragraph as a KG and subsequently requesting ChatGPT-3.5 to predict the missing entity based on the KG, we can observe a more fluent and logical inference process leading to the correct answer.

\begin{tcbraster}[raster equal height,raster valign=top,raster columns=1, raster rows=1, colback=white,colframe=white]
\begin{tcolorbox}[title = Without Prompt Engineering, colback=blue!5!white,colframe=blue!75!black,fonttitle=\bfseries,height=1.5cm]
The Pacific Ocean

\end{tcolorbox}
\begin{tcolorbox}[title = \model{},colback=blue!5!white,colframe=blue!75!black,fonttitle=\bfseries,height=9.6cm]
The question you're asking is: Which of the following is the greatest source of wild fish for human populations? Assuming that the list of possibilities includes the ocean, in triple form, this question would be: \hl{(?, is\_source\_of, wild\_fish)}.

Looking at the given facts:

\hl{(Ocean, is a, Largest body of water on earth)

(Body of water, is a, Source of wild fish for human population)

(Larger body of water, has more, Wild fish)}

Using these facts, we can infer that as the Ocean is the largest body of water on earth and larger bodies of water contain more wild fish, the Ocean would be the greatest source of wild fish for human populations.

\hl{So the answer is: Ocean.}

\end{tcolorbox}

\end{tcbraster}



\textbf{Dynamic KG}: A dynamic KG is designed to incorporate information that changes over time. An example of dynamic KG is given as follows:

``QUESTION: Alice, Bob, and Claire are holding a white elephant gift exchange. At the start of the event, they are each holding a present of a different color: Alice has a yellow present, Bob has a brown present, and Claire has a blue present. As the event progresses, pairs of people swap gifts. First, Bob and Alice swap their gifts. Then, Claire and Alice swap their gifts. Finally, Bob and Alice swap their gifts. At the end of the event, Bob has the
OPTIONS: (A) yellow present (B) brown present (C) blue present'' CORRECT ANSWER: (C). 

It is noticeable that even though the graph itself is uncomplicated, the relationships among individual elements change frequently, posing a challenge for ChatGPT-3.5 to solve. Consequently, without prompt engineering, it provides an incorrect response. However, when we transform the unstructured text into a KG and instructing ChatGPT-3.5 to monitor the changes within the KG, we can observe a comprehensive and precise tracking of changes at each time step, ultimately resulting in the correct answer.


\begin{tcbraster}[raster equal height,raster valign=top,raster columns=1, raster rows=1, colback=white,colframe=white]
\begin{tcolorbox}[title = Without Prompt Engineering ,colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,height=1.5cm]
(B) brown present

\end{tcolorbox}
\begin{tcolorbox}[title = \model{},colback=red!5!white,colframe=red!75!black,fonttitle=\bfseries,height=13cm]
At the start of the event, Alice has a yellow present, Bob has a brown present, and Claire has a blue present. Let's represent this information in a knowledge graph:

Alice - has - yellow present

Bob - has - brown present

Claire - has - blue present

Now, let's go through the swaps step by step and update the knowledge graph accordingly:

\hl{1. Bob and Alice swap their gifts:}

Alice - has - brown present

Bob - has - yellow present

Claire - has - blue present

\hl{2. Claire and Alice swap their gifts:}

Alice - has - blue present

Bob - has - yellow present

Claire - has - brown present

\hl{3. Bob and Alice swap their gifts again:}

Alice - has - yellow present

Bob - has - blue present

Claire - has - brown present

At the end of the event, Bob has the blue present. Therefore, the answer is option (C) blue present.

\end{tcolorbox}

\end{tcbraster}

\subsubsection{Complex Entity Prediction}
The query-answering task shares similarities with entity prediction, but with a key distinction. While entity prediction primarily focuses on one-hop queries in the form of $(e_i, r_k, ?)$ or $(?, r_k, e_j)$, query answering extends the scope to predicting answers for queries with a more complex structure. For example, ``Riom Trial was headed by the French general who reached what distinction?'' is a complex query, which can be expressed in formal logic as $V_? := (\text{Riom Trial}, \text{wasHeadedBy}, V) \land (V, \text{Reached}, V_?)$. The bridging questions in HotpotQA provide typical natural language questions for query answering. They require connecting multiple pieces of information within a document or multiple documents to answer the questions correctly. An instance of bridging questions in HotpotQA is given in Fig.~\ref{fig:Complex Query Answering}. Given that it demands multi-hop sequential reasoning across numerous pieces of information dispersed throughout the extensive article, answering the question poses significant challenges for GPT-3.5 in terms of information gathering and reasoning. Our \model{} addresses this query answering task by structuring the information within the article into a KG, enabling efficient information gathering and reasoning. Additionally, we offer an illustrative example for comparison between GPT-3.5 without prompt engineering and our proposed methods. Due to the article's substantial length and the constraints of space, we have included the example in the appendix.


As it requires multi-hop sequential reasoning over multiple pieces of information to answer the question and these pieces of information are scattered across very distant parts of the long article, which present huge challenges for GPT3.5 to gather information and conduct reasoning. We also provide an example to show 
show how our \model{} help in address query answering task. Since the article is long and we do not have enough space in the main context, we provide it in the appendix. 
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figure/Complex Query Answering.pdf}
    %\vspace{-2em}
    \caption{The bridging question in HotpotQA. It relies on multi-hop sequential reasoning to answer the question. } 
    \label{fig:Complex Query Answering}
\end{figure}

